Improving Mild Cognitive Impairment Prediction via Reinforcement Learning and Dialogue Simulation

Mild cognitive impairment (MCI) is a prodromal phase in the progression from normal aging to dementia, especially Alzheimers disease. Even though there is mild cognitive decline in MCI patients, they have normal overall cognition and thus is challenging to distinguish from normal aging. Using transcribed data obtained from recorded conversational interactions between participants and trained interviewers, and applying supervised learning models to these data, a recent clinical trial has shown a promising result in differentiating MCI from normal aging. However, the substantial amount of interactions with medical staff can still incur significant medical care expenses in practice. In this paper, we propose a novel reinforcement learning (RL) framework to train an efficient dialogue agent on existing transcripts from clinical trials. Specifically, the agent is trained to sketch disease-specific lexical probability distribution, and thus to converse in a way that maximizes the diagnosis accuracy and minimizes the number of conversation turns. We evaluate the performance of the proposed reinforcement learning framework on the MCI diagnosis from a real clinical trial. The results show that while using only a few turns of conversation, our framework can significantly outperform state-of-the-art supervised learning approaches.

==> sec_prob.tex <==
% !TEX root = main.tex

\raggedbottom
\begin{figure}{}
\centering
\includegraphics[width=0.48\textwidth]{fig/fig3.jpg}
\caption{Reinforcement Learning Pipeline.}
\label{fig:fig3}
\end{figure}

The framework we propose in this paper involves the use of reinforcement learning to learn the optimal set of questions to ask patients for the purposes of distinguishing MCI. 
We generate new episodes from these questions for prediction rather than the original corpus. 
Figure \ref{fig:fig3} illustrates our experimental pipeline for our RL framework. The corpus is first preprocessed into distributed vectorized representations ~\cite{mikolov2013distributed,kiros2015skip} to facilitate downstream prediction tasks.
The classifier is trained by supervised learning just like the original supervised framework. 
Once trained, the classifier is then used by the dialogue manager (DM) to train the RL-agent.
In a separate module, an user simulator is trained via supervised learning which outputs distributed representation of patient responses when given various input questions.
Because we want to capture the idiosyncracies of speech behavior for each patient, a separate user simulator is trained over each corpus.
Finally, given the trained RL-agent and user simulator, novel conversational episodes can be produced for test set patients for prediction. 
Our RL + user-simulator modules essentially serve as an additional feature transformation step. 
We will show in the following sections that the synthetic episodes out-perform the original corpus in unseen patients by producing more task-oriented conversational episodes which lend itself to more efficient predictions and data augmentation effects.
